RespireNet: A Deep Neural Network for Accurately Detecting Abnormal Lung Sounds in Limited Data Setting

Auscultation of respiratory sounds is the primary tool for screening and diagnosing lung diseases. Automated analysis, coupled with digital stethoscopes, can play a crucial role in enabling tele-screening of fatal lung diseases. Deep neural networks (DNNs) have shown a lot of promise for such problems, and are an obvious choice. However, DNNs are extremely data hungry, and the largest respiratory dataset ICBHI has only 6898 breathing cycles, which is still small for training a satisfactory DNN model. In this work, RespireNet, we propose a simple CNN-based model, along with a suite of novel techniques -- device specific fine-tuning, concatenation-based augmentation, blank region clipping, and smart padding -- enabling us to efficiently use the small-sized dataset. We perform extensive evaluation on the ICBHI dataset, and improve upon the state-of-the-art results for 4-class classification by 2.2%

==> src/datasets.tex <==
\section{Dataset}

\textbf{ICBHI Dataset:} The ICBHI scientific challenge respiratory sound dataset \cite{icbhi_17, icbhi_19} is one of the largest publicaly available respiratory datasets. The dataset comprises of 920 recordings from 126 patients with a combined total duration of 5.5 hours. Each breathing cycle in a recording is annotated by a single expert as one of the four classes: \textit{normal, crackle, wheeze or both (crackle and wheeze)}. These cycles have various recording lengths\footnote{$65\%$ of the samples have a cycle length of $<3$ seconds, and $33\%$ of the samples have a cyle length between $4-6$ seconds.} ranging from 0.2s to 16.2s (mean cycle length is 2.7s) and the number of cycles is imbalanced across the four classes (i.e. 3642, 1864, 886, 506 cycles for \textit{normal, crackle, wheeze and both} classes respectively). The samples in the dataset were recorded with four different instruments \footnote{AKGC417 L Microphone, 3M Littmann Classic II SE Stethoscope, 3M Litmmann 3200 Electronic Stethoscope and WelchAllyn Meditron Master Elite
Electronic Stethoscope} from hospitals in Portugal and Greece. For every patient, data was recorded from seven different locations in the body.
%: 1) Trachea 2) Anterior left 3) Anterior right 4) Posterior left 5) Posterior right 6) Lateral left and 7) Lateral right. 
The data also contains a significant number of samples which are noisy and were recorded with a wide range of sampling frequencies from 4 kHz to 44.1 kHz. These factors make the problem more challenging and closer to real world scenarios as compared to datasets manually curated under ideal settings, or pure respiratory sound datasets which are used for training professionals (R.A.L.E) \Sid{cite}.

\input{src/tables/per_class_device_wise}

\noindent
\textbf{Critique of the dataset:}
Although the ICBHI challenge does provide the community with a single, largest publicly available dataset for understanding adventitious lung sounds, there are some evident flaws in the dataset. The dataset consists of sound recordings from four devices D1, D2, D3, D4 and is not balanced across patients as well as number of breathing cycles. This creates a skew in the data and has an adverse impact on the performance of the model. This is depicted by our experiment XYZ, and Table \ref{tab:scores_device_wise}. Where the performance of the model across devices is proportional to the distribution of classes within each device.

For creating the splits we perform sample 80-20 w.r.t number of patients. From the numbers in Table \ref{tab:cyles_class_device}, we have 64 patients from Meditron but only 1468 breathing cycles (22.9 breathing cycles per patient on an average), whereas for AKGC417L we have 32 patients and 4364 breathing cycles (136.4 breathing cycles per patient on an average). This does create a huge skew in the splits across devices and patients.
 
Further there is also a skew between abnormal classes across devices: The majority of crackle class (83\% of the total samples) is found within AKGC417L device where is wheeze has a different proportion across devices. This could be another reason for the model overfitting on the abnormal classes during later stages of training (increasing losses during training and still no drop in accuracy).

To overcome this, we propose to first train the model on all the devices to enable it to learn general features and then fine-tune the model for each device separately. This helps in improving the performance and the results are demonstrated in Section or Tables \ref{tab:result_comparison}, \ref{tab:scores_device_wise}.

\Sid{Dataset has served it's purpose, results show that DL methods outperform traditional methods, and we should move in direction of a larger better dataset.}
\Sid{re-write to fit the flow}


==> src/tables/dataset_tables.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c c c c | c}
    \toprule
    \textbf{Normal} & \textbf{Crackle} &\textbf{ Wheeze} & \textbf{Both} & \textbf{Total}  \\
    \cmidrule(lr){1-4}
    \cmidrule(lr){5-5}
    3642 & 1864 & 886 & 506 & 6898 \\
    \bottomrule
    \end{tabular}
    \caption{\textit{Dataset classwise breathing cycles split.}}
    \label{tab:dataset_numbers}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
    \toprule
    \textbf{Diagnosis} & \textbf{Counts}\\
    \hline
    COPD & 64\\
    URTI & 12\\
    LRTI & 2\\
    Bronchiectasis & 7\\
    Bronchiolitis & 6\\
    Pneumonia & 6\\
    Asthma	& 1\\

    \bottomrule
    \end{tabular}
    \caption{\textit{Diagnosis for number of patients.}}
    \label{tab:diagnosis}
\end{table}

\begin{table}[]
    \centering
    \small
    \begin{tabular}{c | c c c c c}
    \toprule
    \textbf{Duration} & \textbf{Normal} & \textbf{ Crackle} & \textbf{Wheeze} & \textbf{Both} & \textbf{Overall}\\
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-6}
    Longest Cycle & 16.2 & 8.7 & 9.2 & 8.6 & 16.2\\
    Shortest Cycle & 0.2 & 0.37 & 0.23 & 0.57 & 0.2\\
    Average Cycle & 2.6	& 2.8	& 2.7	& 3.0 & 2.7\\
    Std-dev Cycle & 1.3 & 0.9 & 1.1 & 1.0 & 1.2\\
    \bottomrule
    \end{tabular}
    \caption{\textit{Duration of cycle length across classes.}}
    \label{tab:duration}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|c}
    \toprule
    \textbf{Duration} & \textbf{Fraction of Samples}\\
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    $<$ 1 second & 0.04\\
    $<$ 2 second & 0.27 \\
    $<$ 3 second & 0.65\\
    $<$ 4 second & 0.88\\
    $<$ 5 second & 0.97\\
    $<$ 6 second & 0.98\\
    \bottomrule
    \end{tabular}
    \caption{\textit{Fraction of samples across different time durations.}}
    \label{tab:duration_fraction}
\end{table}

==> src/tables/dump.tex <==
\begin{table*}[t]
\centering
% \resizebox{\textwidth}{!}{
%\small
\begin{tabular}{ c | c c | c c c}
\toprule
Method & Task & Train$/$Test Split & Spec. & Sen. & Score\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
\cmidrule(lr){4-6}
GMM + HMM \cite{jako_18} &  4-class & 60$/$40 & - & - & 39.5\% \\
X  & 4-class & 60$/$40 & 78.1\% & 20.8\% & 49.4\% \\
Y &  4-class & 60$/$40 & - & - & 49.9\% \\
Z &  4-class & 60$/$40 & 69.2\% & 31.1\% & 50.2\% \\
LungRN+NL &  4-class & 60$/$40 & 63.2\% & 41.3\% & 52.3\% \\
CNN (ResNet34, 6sec) (ours) & 4-class & 60$/$40 & 71.4\% & 39.0\% & 55.2\% \\

\hline

Hybrid CNN-RNN \cite{acharya_20} & 4-class & 80$/$20 & 84.1\% & 48.6\% & 66.3\% \\
LungRN+NL & 4-class & 80$/$20 & 64.7\% & 63.7\% & 64.2\% \\
CNN (ResNet34, 7sec) (ours) & 4-class & 80$/$20 & 78.8\% & 53.6\% & 66.2\% \\
CNN (ResNet34, 7sec) + NewAug (ours) & 4-class & 80$/$20 & 81.7\% & 51.9\% & 66.8\% \\

						
 \bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{Performance comparison of the proposed models with the state of the art systems following random splits.}
% \vspace*{-3mm}
\label{tab:ret_map}
\end{table*}

==> src/tables/results_comparison.tex <==
\begin{table*}[t]
\centering
% \resizebox{\textwidth}{!}{
%\small
\begin{tabular}{ c | c | c | c c c}
\toprule
 & \textbf{Method} & \textbf{Task} & \textbf{Spec}. & \textbf{Sen}. & \textbf{Score}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\textbf{60$/$40 Split} & & & & &\\
& Jakovljevic et al. \cite{jako_18} &  4-class &  - & - & 39.5\% \\
& \citet{chambres_18}  & 4-class & 78.1\% & 20.8\% & 49.4\% \\
& \citet{serbes_18} &  4-class & - & - & 49.9\% \\
& \citet{lungbrn_19} &  4-class & 69.2\% & 31.1\% & 50.2\% \\
& \citet{lungrn_20} &  4-class & 63.2\% & 41.3\% & 52.3\% \\
& CNN (ours) & 4-class & 71.4\% & 39.0\% & \textbf{55.2}\% \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}

\textbf{80$/$20 Split} & & & & &\\
& \citet{noise_rnn_koch_18} & 4-class & 73.0\% & 58.4\% & 65.7 \%\\
& Acharya et al. \cite{acharya_20} & 4-class &  84.1\% & 48.6\% & 66.3\% \\
& \citet{lungrn_20} & 4-class & 64.7\% & 63.7\% & 64.2\% \\
& CNN (ours) & 4-class & 78.8\% & 53.6\% & 66.2\% \\
%& CNN + NA (ours) & 4-class & 81.7\% & 51.9\% & 66.8\% \\
& CNN + NA + BC (ours) & 4-class & 79.7\% & 54.4\% & 67.1\% \\
& CNN + NA + BC + Finetuning (ours) & 4-class & 83.3\% & 53.7\% & \textbf{68.5}\% \\

\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
& CNN (ours) & 2-class & 83.3\% & 60.5\% & 71.9\% \\
& CNN + NA + BC (ours) & 2-class & 76.4\% & 71.0\% & 73.7\% \\
& CNN + NA + BC + Finetuning (ours) & 2-class & 80.9\% & 73.1\% & 77.0\% \\



 \bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{\textit{Performance comparison of the proposed models with the state of the art systems following random splits.}}
% \vspace*{-3mm}
\label{tab:result_comparison}
\end{table*}

==> src/tables/scores_device_wise.tex <==
\begin{table}[]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \small
    \begin{tabular}{c | c | c c c c}
    \toprule
	\textbf{Device} & \textbf{Before$/$After}* & \textbf{N} & \textbf{C} & \textbf{W}	& \textbf{B}\\
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-6}
    AKGC417L & Before & 71.5 & 62.2 & 43.7 & 28.2\\
	AKGC417L & After & 71.2 & 67.3 & 38.4 & 30.7\\

    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-6}

   Meditron & Before & 91.8 & 15.4 & 26.3 & 0\\
   Meditron & After & 92.5 & 15.4 & 36.8 & 0.0\\

    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-6}
    
	Litt3200 & Before & 86.1 & 44.4 & 89.6 & 0\\
	Litt3200 & After & 96.1 & 55.6 &96.5 & 6.7\\
	
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-6}
    
	LittC2SE & Before & 83.9 & 16.7 & 0 & 0\\
	LittC2SE & After & 94.6	& 11.1 & 14.3 & 0.0\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\textit{Scores device wise for each class. This shows that the performance of the class is proportional to the percentage of the samples of that class, present in that device.
    \newline
    *before or after device-specific fine-tuning step.}}
    \label{tab:scores_device_wise}
\end{table}

\begin{table}[]
    \centering
    \resizebox{\linewidth}{!}{
    \small
    \begin{tabular}{c | c | c c c}
    \toprule
	\textbf{Device} & \textbf{\% Samples} & \textbf{Score Before} & \textbf{Score After} & \textbf{Score Improvement} \\
    \cmidrule(lr){1-1}
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-5}
    AKGC417L & 63\% & 60.8\% & 62.5\% & 1.7\%\\

    Meditron & 21\% & 70.1\% & 71.7\% & 1.6\%\\
   
    Litt3200 & 9\% & 81.8\% & 91.1\% & 9.3\%\\

    LittC2SE & 7\% & 50.8\% & 59.4\% & 8.6\%\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\textit{Scores device wise before and after fine-tuning. This shows that the improvement in performance  is proportional to the percentage of the samples of  present in that device.}}
    \label{tab:scores_device_wise}
\end{table}

==> src/tables/time-slice_ablations_old.tex <==
\begin{table}[t]
\centering
% \resizebox{\textwidth}{!}{
%\small
\begin{tabular}{ c | c c }
\toprule
\textbf{Cycle Len.} & \textbf{Task} & \textbf{Score}\\
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}
1 sec & 4-class & 56.6\\
2 sec & 4-class & 59.0\\
3 sec & 4-class & 60.3\\
4 sec & 4-class & 61.1\\
5 sec & 4-class & 62.3\\
6 sec & 4-class & 64.4\\
7 sec & 4-class & \textbf{66.2}\\
8 sec & 4-class & 65.1\\
9 sec & 4-class & 65.5\\


 \bottomrule
\end{tabular}
% }
\vspace{-2mm}
\caption{\textit{Effect of cycle length on the classification performance.}}
% \vspace*{-3mm}
\label{tab:time-slice_ablation}
\end{table}
